A Declarative Validator for GSOS Languages

Rule formats can quickly establish meta-theoretic properties of process algebras. It is then desirable to identify domain-specific languages (DSLs) that can easily express rule formats. In prior work, we have developed Lang-n-Change, a DSL that includes convenient features for browsing language definitions and retrieving information from them. In this paper, we use Lang-n-Change to write a validator for the GSOS rule format, and we augment Lang-n-Change with suitable macros on our way to do so. Our GSOS validator is concise, and amounts to a few lines of code. We have used it to validate several concurrency operators as adhering to the GSOS format. Moreover, our code expresses the restrictions of the format declaratively.

==> eptcsdata.tex <==
\providecommand{\firstpage}{14}
\providecommand{\publicationstatus}{Ilaria Castellani and Alceste Scalas (Ed.): 14th Workshop\\
on Programming Language Approaches to Concurrency and\\ Communication-cEntric Software (PLACES 2023).\\
EPTCS 378, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.378.2}{10.4204/EPTCS.378.2}}

